Halo detection via large-scale Bayesian inference

We present a proof-of-concept of a novel and fully Bayesian methodology designed to detect halos of different masses in cosmological observations subject to noise and systematic uncertainties. Our methodology combines the previously published Bayesian large-scale structure inference algorithm, HADES, and a Bayesian chain rule (the Blackwell-Rao Estimator), which we use to connect the inferred density field to the properties of dark matter halos. To demonstrate the capability of our approach we construct a realistic galaxy mock catalogue emulating the wide-area 6-degree Field Galaxy Survey, which has a median redshift of approximately 0.05. Application of HADES to the catalogue provides us with accurately inferred three-dimensional density fields and corresponding quantification of uncertainties inherent to any cosmological observation. We then use a cosmological simulation to relate the amplitude of the density field to the probability of detecting a halo with mass above a specified threshold. With this information we can sum over the HADES density field realisations to construct maps of detection probabilities and demonstrate the validity of this approach within our mock scenario. We find that the probability of successful of detection of halos in the mock catalogue increases as a function of the signal-to-noise of the local galaxy observations. Our proposed methodology can easily be extended to account for more complex scientific questions and is a promising novel tool to analyse the cosmic large-scale structure in observations.

==> BlackwellRaoEstimator.tex <==
\appendix

\section{Bayesian translation between density and halo mass}
\label{sec:build_joint_prob}

Suppose we would like to know how likely it is to find the mass of the
most massive halo in a voxel centred at a redshift $z$ with a given
value of the density field, $\delta$. In Bayesian parlance we would
like to estimate the probability $\mathcal{P}(M_{{\rm halo}}>M_{{\rm
th.}}|\delta, z)$ of finding the mass $M_{{\rm halo}}$ of the most
massive halo above a threshold mass $M_{{\rm th.}}$, given a value of
the density field $\delta$ at a given redshift $z$.

This probability can be calibrated by N-body simulations via the
following procedure. The first step is to estimate the joint
probability distribution,
\begin{equation}
\mathcal{P}(M_{{\rm halo}},\delta| z),
\end{equation}
for each snapshot of the simulation. This can be done for a single
snapshot in the following way:
\begin{enumerate}
  \item Build a density field from the snapshot at the same grid
  resolution as used for the inference. This can be achieved via a
  Cloud-in-Cell (CiC) procedure.
  \item Allocate a 2-dimensional array with axes corresponding to the
  values of $M_{{\rm halo}}$ and $\delta$.
  \item Loop through the density field constructed via CiC from the
  snapshot. At every voxel estimate the pairs $\{M_{{\rm
  halo}},\delta\}$ of all halo masses of halos whose centre belong to
  that voxel and the density value of that voxel.
  \item Build the 2-dimensional histogram of the pairs $\{M_{{\rm
  halo}},\delta\}$.
\end{enumerate}
The resulting 2-dimensional histogram is an estimate for the joint
probability,
\begin{equation}
\mathcal{P}(M_{{\rm halo}},\delta| z),
\end{equation}
at that particular redshift.

The conditional probability of finding that the most massive halo has a
given mass in a given voxel with density $\delta$ is then:
\begin{equation}
\mathcal{P}(M_{{\rm halo}}|\delta, z)=\frac{\mathcal{P}(M_{{\rm halo}},\delta| z)}{\mathcal{P}(\delta| z)}.
\end{equation}
To determine the conditional probability of the most massive halo
being greater than some threshold value, we can marginalise over all halo masses above the thresold, i.e.
\begin{equation}
\mathcal{P}(M_{{\rm halo}}>M_{{\rm th.}}|\delta, z) = \sum_{M>M_{{\rm th.}}}\mathcal{P}(M_{{\rm halo}}|\delta, z).
\end{equation}

Now we would like to answer the question: ``What is the probability,
given some observations, of that the most massive halo at a given
position in the sky has a mass above a particular threshold value?''
In other words, we would like to evaluate the probability,
$\mathcal{P}(M_{{\rm halo}}>M_{{\rm th.}}|d,z)$. The \HADES{}
framework permits to do this using Blackwell-Rao estimators. In
particular we can calculate the above probability distribution as a
marginalization over all HADES samples,
\begin{eqnarray}
\mathcal{P}(M_{{\rm halo}}|d,z) &=&\int \mathrm{d}\delta \mathcal{P}(M_{{\rm halo}}>M_{{\rm th.}},\delta| d, z) \nonumber \\
&=& \int \mathrm{d}\delta \mathcal{P}(M_{{\rm halo}}>M_{{\rm th.}}|\delta, z)\, \mathcal{P}(\delta|d) \nonumber \\
&=& \frac{1}{N_{\mathrm{samp}}}\sum_{i}^{N_{\mathrm{samp}}} \mathcal{P}(M_{{\rm halo}}>M_{{\rm th.}}|\delta_i, z),
\end{eqnarray}
which in practice is a simple sum over all \HADES{} realizations and
returns a detection probability of finding halos above a given mass at
given positions in the survey. Note that the procedure can be extended
to arbitrary complexity, as all we would need to do is to calibrate
the correponding probability functions from simulations.
